All Your Location are Belong to Us: Breaking Mobile Social Networks for Automated User Location Tracking

Many popular location-based social networks (LBSNs) support built-in location-based social discovery with hundreds of millions of users around the world. While user (near) realtime geographical information is essential to enable location-based social discovery in LBSNs, the importance of user location privacy has also been recognized by leading real-world LBSNs. To protect user's exact geographical location from being exposed, a number of location protection approaches have been adopted by the industry so that only relative location information are publicly disclosed. These techniques are assumed to be secure and are exercised on the daily base. In this paper, we question the safety of these location-obfuscation techniques used by existing LBSNs. We show, for the first time, through real world attacks that they can all be easily destroyed by an attacker with the capability of no more than a regular LBSN user. In particular, by manipulating location information fed to LBSN client app, an ill-intended regular user can easily deduce the exact location information by running LBSN apps as location oracle and performing a series of attacking strategies. We develop an automated user location tracking system and test it on the most popular LBSNs including Wechat, Skout and Momo. We demonstrate its effectiveness and efficiency via a 3 week real-world experiment with 30 volunteers. Our evaluation results show that we could geo-locate a target with high accuracy and can readily recover users' Top 5 locations. We also propose to use grid reference system and location classification to mitigate the attacks. Our work shows that the current industrial best practices on user location privacy protection are completely broken, and it is critical to address this immediate threat.

==> Threat.tex <==
\section{Attack Model}
In this study, we consider a capability-restricted attacker, who aims at geo-locating an LBSN user, who does not need to have a priori social association with me, i.e., an in-app friend. The attacker's capability is restricted in sense that i) It only has the access right no more than a normal user of a given LBSN service, which means that it can only access the publicly available information provided by the LBSN app. ii) it is not allowed to hack the LBSN service by interfering its internal operations, that is, we do not consider an attacker that can compromise the LBSN servers and thus can directly access the user location information as a consequence. In summary, our attacker is a very weak one which can't gain any additional information from the LBSN services other than what is entitled to a regular service user. Specifically, the attacker will try to infer a user's location information based only on the relative distance information displayed by the LBSN apps. Note that, to obtain the relative distance, it is even not necessary for the attacker to be the friend of the victim. In stead, it will automatically display the relative distance of nearby users in most of considered category II apps. For Momo and SKout, the distance between the victim user and the attacker can always be displayed as long as the attacker has sent the message to the victim before. We assume a capability-restricted attacker to examine the security protection strength of the real-world LBSN services. In fact, the attacker we assume is simply a regular user of LBSNs in term of capability. The reasoning behind this strategy is that if the LBSN under examination can't resist even such a weak attacker, the user's location privacy is obviously in a great danger as any user can be an attacker.

We further distinguish two different types of attackers, i.e., a Casual Attacker and a Determined Attacker. A Casual Attacker reviews the profiles of nearby users when login to a LBSN app as a regular user, randomly picks up a tracking target and then try to localize the target.  A Determined Attacker may start with a known User ID (ID) and/or User Number as its chosen attacking target.  Or a Determined Attacker may start with a target person in mind and exploit certain side-channel information of the target to help obtain the corresponding UID or user number. For example, user photos shared among various social network sites can be used to establish the linkage for the same user, which in turn can lead to the acquisition of UID/ User number information in a particular LBSN. Social engineering approaches like this have been wide studied in the literature and is not a focus of this paper. We assume that a Determined Attacker will be able to start with a chosen UID or user number against it wants to localize.




%  In some apps such as skout or Momo, it
%  provides the relative distance of the target and attacker in a large
%  area (even cross the pacific). So it enables the attacker to
%  actively track a target even when they are physically far away.
%
%\item{Stage II.b: Shadow Tracker (Determined, Active Tracker which
%    virtually follows the objective)} For wechat and other apps, which
%  only provides the relative distance in a small area, the attacker
%  could enhance his tracking capability by predicting users' mobility
%  and then follow them. As long as the attacker could always be close
%  to the victim, the attacker can track the victim in a larger area.

%\end{itemize}


%In our attacker model, the attacker aims to compromise the victim's
%location privacy. In the real-world applications, we distinguish the
%attackers into a casual geolocator and a determined tracker. Further,
%a determined tracker could be further classified into long distance
%tracker, for apps providing the relative distance in a large area, and
%shadow tracker, for apps only providing the relative distance in a
%small area. We introduce the capability of various kinds of attackers
%as follows:


==> discussion.tex <==
\subsection{Comparison of Tracking Difficulty}
It is interesting to compare the difficulty of tracking the above 3
popular LBSN apps. In our phase I experiments (or synchronous
tracking), though varying at different localization accuracy, all of
the apps show a high detection successful rate, which is defined as
the rate of successfully launching a localization towards a specific
user. However, In phase II experiment (or asynchronous tracking), it
is observed that there is a certain number of failures on tracking
Wechat user. There are several factors which lead to a high detection
failure rate. Firstly, as the app with coverage limitation, our
experiment only covers an area of a certain size (or Minghang Campus
of Shanghai Jiao Tong University). Our tracking will fail if a
volunteer leaving this area. Secondly, in Wechat, the user's location
information will be kept for a certain duration. This duration varies
at different areas with different user population. Such a cache
duration has no impact on the detection successful rate for phase I
experiments while has a significant impact on the phase II
experiments. During the asynchronous tracking, if the delay between
the user checking in the app and the attack triggered, the track will
fail due to fail to find the target. Therefore, reducing the interval
of launching the tracking will help increase the detection successful
rate. In our experiment, we propose an enhanced hot spot based
scanning approach which could significantly increase the scanning
speed and thus could improve our detection successful rate.

\subsection{Economic Factor of The Attack}
The main part of FreeTrack is written in Clojure, which is a freely available host language on JVM. It depends on Octave and Android SDK, which are another 2 cross-platform projects. The
Android X86 image is hosted on VirtualBox, an open-source virtual
machine. Thus, FreeTrack does not require any specific platform to
run. Each Android X86 image approximately requires 2G hard-drive space
and 1G memory. As most of the running time is spent on waiting the app
server's response, FreeTrack requires extremely low CPU resources and
the only bottleneck is network speed and memory. For a general
discussion, for a PC with quad cores and 8G memory, which is worthy of
600 dollars, it is able to run at least 6-7 instances of FreeTrack. In
our experiments, 3 instances of FreeTrack are sufficient to track 40
Momo users for every 40 mins.  For WeChat, in sparsely populated area,
we use 4 nodes to cover the whole downtown of Buffalo and in densely
populated area like Shanghai, the Lujiazui could be covered with 28
nodes under extreme conditions but generally, 5-7 nodes is sufficient
to handle 15 users. For Skout,........................... In general,
FreeTrach incurs a low hardware cost per a tracking target.

It is also important to point out that, FreeTrack may incur some additional costs
during the running time. For example, for Wechat, it has a strict
restriction on the number of location reports during a specific period in
order to relieve the server load. If exceeding this limit, the Wechat
account will be banned. During our 3 week experiments, 36 WeChat
accounts get banned in China while no accounts are banned in United
States. Registering a WeChat account only takes less than a minute and
buying an account only costs 0.01 USD. Thus, the total cost of
$36$ WeChat accounts is less than 0.6 USD. For Skout, it takes only
about 15 seconds to leave a message to a user and add him into the
targets list. For Skout, to add a user into tracking targets, the best way is to throw a Winked Bomb, for
which every 50 bombs cost 4.99 dollars and is able to bring (how many?!) users into attacking targets.
In summary, the cost during the run time to launch the attack is also very low.

\subsection{Global Tracking or Metropolitan Area Tracking} Due to no display coverage
limitations, Skout and Momo could naturally support Global Tracking, which means a skout user
in China could even freely track a skout user in US by using FreeTack, and vice versa. This may potentially
pose a significant threat to location privacy of mobile users. Duo to the coverage limitation,
it seems difficult to deploy a very large scale tracking coverage in Wechat. However, by jointly
considering technical and economic factors, it is feasible for the attacker to deploy a metropolitan area tracking system as long as it could obtain enough computation, storage and bandwidth resources. The emergence of
cloud based outsourcing or crowdsourcing makes it possible for the attacker to obtain enough resources
in a short time.

\subsection{The Impact of High-granularity Tracking on Re-identification} In our experiments, FreeTrack shows a
fundamental difference with the previous Dataset based location privacy studies (e.g., ) that we could achieve
a high-granularity tracking. Though existing works show that coarse datasets provide little anonymity [], none of
the existing works studies the impact of high-granularity tracking on anonymity. In our study, it is found that
tracking at a very high accuracy will give the attacker a significant advantage in that it could map the tracked location to a specific location or building, which could provide useful side information to re-identify the victim. In the experiment, we could accurately geo-locate a target to SEIEE building, which gives us a high confidence that the target may be the students of school of Electronic, Information and Electrical Engineering and he is using LBSN apps in
his lab.

%
% Nowadays cloud host virtual machines like EC2 may as well be used to
% largely scale the capability of FreeTrack.
%
% In the anonymous trace collection part, we use 3 nodes to track 40
% Momo users every 40 minutes with only assumption that the users are
% in Shanghai. For WeChat, in sparsely populated area, we use 4 nodes
% to cover the whole downtown of Buffalo and in densely populated area
% like Shanghai, the Lujiazui could be covered with 28 nodes under
% extreme conditions but generally, 5-7 nodes is sufficient to handle
% 15 users. Note that Tencent has strict restrictions on number of
% location reports during a time period in order to relieve the server
% load, such restriction appears different with user density as in
% Buffalo, the WeChat number never gets banned for 3 weeks period of
% evaluation but in Shanghai, we have lost 36 WeChat accounts. But to
% register a WeChat account only take less than a minute and buy an
% account from online only costs 0.1 RMB. Thus, the total cost of 36
% WeChat accounts is less than 0.6 dollars. For Skout, to add a user
% into tracking targets, the best way is to throw a Winked Bomb, for
% which every 50 bombs cost 4.99 dollars and is able to bring (how
% many?!) users into attacking targets.

%\subsection{Implication of Accurate Tracking}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mobi_loc"
%%% End:

